Binary Classification Under $\ell_0$ Attacks for General Noise Distribution

Adversarial examples have recently drawn considerable attention in the field of machine learning due to the fact that small perturbations in the data can result in major performance degradation. This phenomenon is usually modeled by a malicious adversary that can apply perturbations to the data in a constrained fashion, such as being bounded in a certain norm. In this paper, we study this problem when the adversary is constrained by the $\ell_0$ norm; i.e., it can perturb a certain number of coordinates in the input, but has no limit on how much it can perturb those coordinates. Due to the combinatorial nature of this setting, we need to go beyond the standard techniques in robust machine learning to address this problem. We consider a binary classification scenario where $d$ noisy data samples of the true label are provided to us after adversarial perturbations. We introduce a classification method which employs a nonlinear component called truncation, and show in an asymptotic scenario, as long as the adversary is restricted to perturb no more than $\sqrt{d}$ data samples, we can almost achieve the optimal classification error in the absence of the adversary, i.e. we can completely neutralize adversary's effect. Surprisingly, we observe a phase transition in the sense that using a converse argument, we show that if the adversary can perturb more than $\sqrt{d}$ coordinates, no classifier can do better than a random guess.

==> app_converse_old.tex <==
\section{Proof of Theorem~\ref{thm:converse}}
\label{app:converse-proof}


{\color{red}[check which of the 4 assumptions I exactly need here and update the
  statement (for now I am including all 4 assumptions to be on the safe side)]}


\newcommand{\xprv}{X_+}
\newcommand{\xmrv}{X_-}

Define the random variable $\xprv$ as $Z + \mu_d$ where $Z \sim \nd(.)$. In
fact, the distribution of $\xprv$  is the same as that of a data sample
conditioned on $Y = +1$. Similarly, define $\xmrv$ as $Z - \mu_d$. Let $(\xprv,
\xmrv)$ be a maximal coupling between $\xprv$ and $\xmrv$ that minimizes
$\pr{\xprv \neq \xmrv}$\footnote{Note that $(Z+\mu_d, Z - \mu_d)$ where $Z \sim
  \nd(.)$ is probably not the optimal coupling since $\pr{X_+ \neq X_-} = 1$ unless
  $\mu_d = 0$.}. Given such a maximal coupling, let
\begin{equation*}
  W :=
  \begin{cases}
    \xprv & \text{if } \xprv = \xmrv, \\
    0 & \text{otw}.
  \end{cases}
\end{equation*}
Moreover, let $Y \sim \text{Unif}(\pm 1 )$ be independent from $(X_+, X_-, W)$
and define
\begin{equation*}
  X :=
  \begin{cases}
    X_+ & Y = +1 \\
    X_- & Y = -1.
  \end{cases}
\end{equation*}
It is easy to verify that $(X,Y)$ have the same joint distribution as our true
feature vector-label pair, i.e.\ for $a \in \reals$ we have 
\begin{equation*}
  \pr{X \leq a | Y = +1} = \pr{X_+ \leq a} = \pr{Z + \mu_d \leq a},
\end{equation*}
and
\begin{equation*}
  \pr{X \leq a | Y = -1} = \pr{X_- \leq a} = \pr{Z - \mu_d \leq a}.
\end{equation*}


% {\color{red}[I am sloppy in this appendix regarding densities / using delta
%   notation etc.]}

% {\color{red}[Also, I am not very consistent regarding random variable
%   (capital/non-capital) notation]}

% Given $X,Y$ such that $Y \sim \text{Unif}(\pm 1)$ and $X = \mu_d Y + Z$ where $Z
% \sim \nd(.)$, define $\tW$ as follows:
% \begin{enumerate}
% \item $\tW$ conditioned on $Y = +1$ and $X = x$ has the same distribution as $W$
%   conditioned on $\xprv = x$, i.e. $f_{\tW | X = x, Y = +1}(.) \equiv f_{W |
%     \xprv = x}(.)$.
% \item $\tW$ conditioned on $Y = -1$ and $X = x$ has the same distribution as $W$
%   conditioned on $\xmrv = x$, i.e. $f_{\tW | X = x, Y = -1}(.) \equiv f_{W |
%     \xmrv = x}(.)$.
% \end{enumerate}

Keep in mind that the joint distribution of $(X_+, X_-, W, Y, X)$ depend on $\mu_d$ and hence on $d$. However, we do not make such a dependence
explicit to simplify the notation.

The following lemma, whose proof is given at the end of this section, shows that
$\tW$ is independent from $Y$.

\begin{lem}
  \label{lem:tW-indep-Y}
  $\tW$ is independent from $Y$. 
\end{lem}

Note that by definition, $W$ is a function of $(X_+, X_-)$ and hence is
independent from $Y$. 
This suggests that $W$ can be considered as a good candidate for the
adversary's perturbation, since the adversary would ideally like to perturb the
data in a way that the information about the true label is removed. More
precisely, given the true label $y$ and data samples $(\xd_i: i \in [d])$, we
generate the modified data samples $\vtwd = (\twd_i: i \in [d])$ such that $\twd_i$ are
conditionally independent conditioned on $y$, and $\twd_i$ is generated from the
law of $\tW$ conditioned on $Y=y$ and $X = \xd_i$. Lemma~\ref{lem:tW-indep-Y}
above ensures that the modified samples $\twd_i$ do not bear any information
about the label $y$, however $\snorm{\vtwd - \vxd}_0$ might be above the
adversary's budget $k_d$. In order to address this, we define the final
perturbed data vector $\vxpd$ as follows:
\begin{equation}
  \label{eq:lower-bound-vxpd}
  \vxpd =
  \begin{cases}
    \vtwd & \text{if } \snorm{\vtwd - \vxd}_0  \leq k_d \\
    \vxd & \text{otw.}
  \end{cases}
\end{equation}
This ensures that indeed $\snorm{\vxpd - \vxd}_0 \leq k_d$. In fact, it turns
out that if $k_d \gg \sqrt{d}$, then $\snorm{\vtwd - \vxd}_0 \leq k_d$ with high
probability. The following lemma,  will be later useful to make this statement
precise. The proof of Lemma~\ref{lem:adv-modification-expectation} below is given at the end of this section.

\begin{lem}
  \label{lem:adv-modification-expectation}
  Assume that the Assumption~\ref{assumption:Fisher} is satisfied and $\mu_d = c
  / \sqrt{d}$ for some $c > 0$. Then for any
  $\delta > 0$ we have
  \begin{equation*}
    \lim_{d \rightarrow \infty} \frac{\pr{\tW \neq X| Y = +1}}{d^{-\frac{1}{2} + \delta}} = 0,
  \end{equation*}
  and
    \begin{equation*}
    \lim_{d \rightarrow \infty} \frac{\pr{\tW \neq X| Y = -1}}{d^{-\frac{1}{2} + \delta}} = 0.
  \end{equation*}
\end{lem}

% see gtag 2022-01-11 11-03-50

\begin{proof}[Proof of Theorem~\ref{thm:converse}]
  Assume that the adversary employs the above strategy to perturb the input
  samples. In order to obtain a lower bound for the optimal robust error
  $\optroberrd_{\mu_d, \nd(.)}(k_d)$, we consider any classifier $\mC$, and further
  assume that the classifier knows adversary's budget (hence making the
  classifier stronger, yielding a lower bound). Note that upon observing
  $\vxpd$, if the conditional densities $f_{\vxpd|y=+1}(\vxpd)$ and
  $f_{\vxpd|y=-1}(\vxpd)$ are the same, the classifier cannot do better than a
  random guess. Hence, we have
  \begin{equation}
    \label{eq:converse-l-C-equal-dens-1}
\begin{aligned}
  \roberrd_{\mu_d, \nd(.)}(\mC, k_d) &\geq \frac{1}{2} \pr{f_{\vxpd|y=+1}(\vxpd) = f_{\vxpd|y=-1}(\vxpd)} \\
  &= \frac{1}{4} \pr{f_{\vxpd|y=+1}(\vxpd) = f_{\vxpd|y=-1}(\vxpd) | y = +1} \\
  &\qquad + \frac{1}{4} \pr{f_{\vxpd|y=+1}(\vxpd) = f_{\vxpd|y=-1}(\vxpd) | y = -1}.
\end{aligned}
\end{equation}
Let $I$ be the indicator of the event $\snorm{\vtwd - \vxd}_0 > k_d$. We may
write
\begin{equation*}
%\label{eq:converse-pr-equal-density-1}
\begin{aligned}
  &\pr{f_{\vxpd|y=+1}(\vxpd) = f_{\vxpd|y=-1}(\vxpd) | y = +1} \\
  &\qquad \geq \pr{f_{\vxpd|y=+1}(\vxpd) = f_{\vxpd|y=-1}(\vxpd), I = 0 | y = +1}\\
  &\qquad \stackrel{(a)}{=} \pr{f_{\vtwd|y=+1}(\vtwd) = f_{\vtwd|y=-1}(\vtwd), I = 0 | y = +1} \\
  &\qquad = \pr{f_{\vtwd|y=+1}(\vtwd) = f_{\vtwd|y=-1}(\vtwd) | y = +1} - \pr{I = 1|y=+1} \\
  &\qquad \stackrel{(b)}{=} 1 - \pr{I = 1 | y=+1}
\end{aligned}
\end{equation*}
where $(a)$ uses the fact that when $I = 0$, $\vxpd = \vtwd$ by definition, and
$(b)$ uses the fact that from Lemma~\ref{lem:tW-indep-Y}, $\vtwd$ is independent
from $y$. This together with a similar bound conditioned on $y=-1$ together
with~\eqref{eq:converse-l-C-equal-dens-1} implies that
\begin{equation*}
  \roberrd_{\mu_d, \nd(.)}(\mC, k_d) \geq \frac{1}{2} - \frac{1}{4} \left( \pr{I = 1|y=+1} + \pr{I = 1|y=-1} \right).
\end{equation*}
Since this inequality holds for any classifier $\mC$, we get
\begin{equation}
  \label{eq:converse-lstar-bound-1}
  \optroberrd_{\mu_d, \nd(.)}(k_d) \geq \frac{1}{2} - \frac{1}{4} \left( \pr{I = 1|y=+1} + \pr{I = 1|y=-1} \right).
\end{equation}
We now argue that $\pr{I = 1|y=+1}$ and $\pr{I = 1|y=-1}$ vanish as $d
\rightarrow \infty$, provided that $k_d \geq d^{1/2 + \epsilon}$. We give the
proof for $\pr{I = 1|y=+1}$, since the other term vanishes with a similar
argument. Let $I_i, 1 \leq i \leq d$ be the indicator that $\twd_i \neq \xd_i$.
Using Markov inequality together with
Lemma~\ref{lem:adv-modification-expectation}, we have
\begin{align*}
  \pr{I = 1|y = +1} &= \pr{\sum_{i=1}^d I_i> k_d | y = +1} \\
                    &\leq \frac{d \pr{\tW \neq X | Y = +1}}{k_d} \\
                    &\leq \frac{d \pr{\tW \neq X | Y = +1}}{d^{1/2 + \epsilon}} \\
                    &= \frac{\pr{\tW \neq X | Y = +1}}{d^{-1/2 + \epsilon}},
\end{align*}
which goes to zero as $d \rightarrow \infty$ due to
Lemma~\ref{lem:adv-modification-expectation}. Using a similar argument
conditioned on $y=-1$ and substituting in~\eqref{eq:converse-lstar-bound-1}, we
realize that $\liminf_{d \rightarrow \infty} \optroberrd_{\mu_d, \nd(.)}(k_d)
\geq 1/2$, which completes the proof.
\end{proof}

\begin{proof}[Proof of Lemma~\ref{lem:tW-indep-Y}]
  We have
  \begin{align*}
    f_{\tW | Y = +1}(\tw) &= \int f_{\tW | X = x, Y = +1}(\tw) f_{X | Y = +1}(x_+) dx_+ \\
                          &\stackrel{(a)}{=} \int f_{W | \xprv = x_+}(\tw) f_{\xprv}(x_+) dx_+ \\
                          &= \int f_{W, \xprv}(\tw, x_+) dx_+ \\
                          &= \int f_{W, \xprv, \xmrv} (\tw, x_+, x_-) dx_+ dx_- \\
                          &= \int_{x_+ = x_-} f_{W, \xprv, \xmrv} (\tw, x_+, x_-) dx_+ dx_- \\
                          &\qquad + \int_{x_+ \neq x_-} f_{W, \xprv, \xmrv} (\tw, x_+, x_-) dx_+ dx_- \\
                          &= \int_{x_+ = x_-} f_{\xprv, \xmrv} (x_+, x_-) \delta(\tw - x_+)dx_+ dx_- \\
                          &\qquad + \int_{x_+ \neq x_-} f_{\xprv, \xmrv} (x_+, x_-) \delta(\tw - 0)dx_+ dx_- \\
    &= f_{\xprv, \xmrv}(\tw, \tw) + \pr{\xprv \neq \xmrv} \delta(\tw - 0).
  \end{align*}
  where $(a)$ uses the definition of $\tW$ and the fact that $\xprv$ has the
  same distribution as $X$ conditioned on $Y = +1$. A similar calculation shows
  that
  \begin{equation*}
    f_{\tW | Y = -1}(\tw) = f_{\xprv, \xmrv}(\tw, \tw) + \pr{\xprv \neq \xmrv} \delta(\tw - 0),
  \end{equation*}
  and completes the proof.
\end{proof}

\begin{proof}[Proof of Lemma~\ref{lem:adv-modification-expectation}]
  {\color{red}to be added.}
\end{proof}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:

